Estimating the Local Air Pollution Impacts of Maritime Traffic: A Principled Approach for Observational Data

We propose a new approach to estimate the causal effects of maritime traffic when natural or policy experiments are not available. We apply this method to the case of Marseille, a large Mediterranean port city, where air pollution emitted by cruise vessels is a growing concern. Using a recent matching algorithm designed for time series data, we create hypothetical randomized experiments to estimate the change in local air pollution caused by a short-term increase in cruise traffic. We then rely on randomization inference to compute nonparametric 95\% uncertainty intervals. We find that cruise vessels' arrivals have large impacts on city-level hourly concentrations of nitrogen dioxide, particulate matter, and sulfur dioxide. At the daily level, road traffic seems however to have a much larger impact than cruise traffic. Our procedure also helps assess in a transparent manner the identification challenges specific to this type of high-frequency time series data.

==> tables/new_table_matching_results.tex <==
\begin{table}[h!]
\caption{Number of Matched Pairs by Experiment.}\label{matching_results}
\begin{threeparttable}
\begin{tabularx}{\textwidth}{Xcc}
\toprule
& \textbf{\shortstack{Hourly \\ cruise arriving}} 
& \textbf{\shortstack{Daily \\ cruise arriving}}  \\ \midrule
\rowcolor{Gray}
N$_{\mathrm{Total}}$ &  96,432  & 4,018  \\
N$_{\mathrm{Treated}}$ &  4,034   & 1,081   \\
\rowcolor{Gray}
N$_{\mathrm{Control}}$ & 92,396   & 1,619 \\
N$_{\mathrm{Pairs}}$   & 138   & 209   \\
\bottomrule
\end{tabularx}
\begin{tablenotes}
\footnotesize
\item \textit{Notes}: This table displays the total number of observations, N$_{\mathrm{Total}}$ for each experiment, the number of potential treated and controls units before matching, N$_{\mathrm{Treated}}$ and N$_{\mathrm{Control}}$, and the number of matched pairs, N$_{\mathrm{Pairs}}$.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/new_table_matching_thresholds.tex <==
\begin{table}[h!]
\footnotesize
\caption{Maximum Discrepancies allowed for each Covariate between Treated and Control Units, Hourly and Daily Experiments.}\label{tab_thresholds}
\begin{threeparttable}
\begin{tabularx}{\textwidth}{Xcc}
\toprule
& \textbf{\normalsize Hourly Experiment} & \textbf{\normalsize Daily Experiment} \\ \midrule
\multicolumn{3}{@{}l}{\textbf{\normalsize Calendar Indicators}}\\
\rowcolor{Gray}
Distance in days                               & 30              & 1095               \\
Hour of the day in \textit{t}   & 0               &               \\
Weekday, Bank Days and Holidays in \textit{t}   & 0               & 0              \\
\rowcolor{Gray}
Weekday, Bank Days and Holidays in \textit{t-1} & 0               & 0              \\
Weekday, Bank Days and Holidays in \textit{t-2} & 0               &                \\
\rowcolor{Gray}
Month in \textit{t}                                      &           & 0 \\
\rowcolor{Gray}
\midrule
\multicolumn{3}{@{}l}{\textbf{\normalsize Weather Parameters}}\\
Average Temperature (°C) in \textit{t}                       & 4               & 4              \\
\rowcolor{Gray}
Average Temperature (°C) in \textit{t-1}                     & 4               & 4              \\
Average Temperature (°C) in \textit{t-2}                     & 4               &                \\
\rowcolor{Gray}

Rainfall Dummy in \textit{t}                            & 0               & 0              \\
Rainfall Dummy in \textit{t-1}                         & 0               & 0              \\
\rowcolor{Gray}

Rainfall Dummy in \textit{t-2}                          & 0               &                \\
Average Humidity (\%) in \textit{t}                          & 9               &              \\
\rowcolor{Gray}

Average Humidy (\%) in \textit{t-1}                         & 9               &              \\
Average Humidity (\%) in \textit{t-2}                        & 9               &                \\
\rowcolor{Gray}

Wind direction in 2 categories (East/West) \textit{t}                  & 0            &  0        \\
Wind direction in 2 categories (East/West) \textit{t-1}                  & 0            & 0           \\
\rowcolor{Gray}
Wind direction in 2 categories (East/West) \textit{t-2}                  & 0            &               \\ 
Wind speed (m/s) in \textit{t}                                & 1.8  & 2 \\
\rowcolor{Gray}
Wind speed (m/s) in \textit{t-1}                               & 1.8 & 2 \\
Wind speed (m/s) in \textit{t-2}                               & 1.8 &  \\
\bottomrule
\end{tabularx}
\begin{tablenotes}
\footnotesize
\item \textit{Notes}: This table displays the maximum distance allowed for each covariate in the pair matching algorithm, for each experiment. For example, it means that, for each matched pair, treated and control units must have the same values for weekday, bank days and holidays indicators in \textit{t}. If a discrepancy value is missing in one of the two column, it means that the associated covariate was not used for matching for the corresponding experiment.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/table_descriptive_stat.tex <==
\begin{table}[h!]
\footnotesize
\caption{Descriptive statistics at the daily level (2008-2018)}\label{table_descriptive_statistics}
\begin{threeparttable}
\begin{tabularx}{\textwidth}{Xcccc}
\toprule
\textbf{Variable}            & \textbf{Mean} & \textbf{Standard Deviation} & \textbf{Minimum} & \textbf{Maximum} \\ \midrule
\multicolumn{5}{@{}l}{\textbf{\normalsize Vessel traffic}}\\
\rowcolor{Gray}
Total Entering and Exiting Gross tonnage (unitless) & 581,245 & 260,705 & 34,325 & 1,691,428 \\
Number of Vessel entrances & 10.2 & 3.3 & 1 & 23 \\
\rowcolor{Gray}
Total Entering and Exiting Cruise Gross tonnage (unitless) & 189,700 & 231,796 & 0 & 1,245,396 \\
Number of Cruise Vessel entrances & 1.4 & 1.4 & 0 & 11 \\
\rowcolor{Gray}
Total Entering and Exiting Ferry Gross tonnage (unitless) & 279,470  & 101,431 & 0 & 663,733 \\
Number of Ferry Vessel entrances & 4.7 & 1.9 & 0 & 11 \\
\multicolumn{5}{@{}l}{\textbf{\normalsize Pollution}}\\
\rowcolor{Gray}
NO$_{2}$ ($\mu g/m^{3}$)  at Longchamp   & 30.0         & 13.3                     & 4.0              & 93.0\\
NO$_{2}$ ($\mu g/m^{3}$)  at Saint-Louis   & 36.5         & 16.4                     & 3.0              & 91.0\\
\rowcolor{Gray}
O$_{3}$ ($\mu g/m^{3}$) at Longchamp     &   53.8        &      23.1                  &       2         &   121\\
PM$_{10}$ ($\mu g/m^{3}$) at Longchamp    & 26.9         & 10.7                        & 5.0              & 114.0            \\
\rowcolor{Gray}
PM$_{10}$ ($\mu g/m^{3}$) at Saint-Louis    & 30.4         & 15.3                        & 3.0              & 176.0            \\
PM$_{2.5}$ ($\mu g/m^{3}$) at Longchamp   & 15.4          & 8.5                         & 0                & 77.0             \\
\rowcolor{Gray}
SO$_{2}$ ($\mu g/m^{3}$) at Longchamp    & 2.3           & 2.5                         & 0                & 32.0             \\
\multicolumn{5}{@{}l}{\textbf{\normalsize Weather}}\\
\rowcolor{Gray}
Average Temperature (°C)     & 15.9          & 7.0                         & -3.5             & 31.3             \\
Average Rainfall Height (mm) & 1.6           & 5.9                         & 0                & 104.2            \\
\rowcolor{Gray}
Average Humidity (\%)        & 65.2          & 12.4                        & 30               & 96               \\
Wind Speed (m/s)             & 4.7           & 2.8                         & 0.4              & 17.8   \\
\multicolumn{5}{@{}l}{\textbf{\normalsize Health}}\\
\rowcolor{Gray}
Emergency admissions for Circulatory or Respiratory causes$^{a}$          & 29.6 & 9.4 & 7 & 74 \\
Death count for Non-Accidental Causes$^{b}$                       & 21.7 & 5.3                & 7       & 43      \\
\rowcolor{Gray}
Death count for Non-Accidental Causes (Age $\geq$ 75)$^{b}$ & 15.3 & 4.4                & 4       & 36      \\
Death count for Circulatory Causes$^{b}$                        & 5.9  & 2.7                & 0       & 16      \\
\rowcolor{Gray}
Death count for Circulatory Causes (Age $\geq$ 75)$^{b}$    & 4.8  & 2.3                & 0       & 14      \\
Death count for Respiratory Causes$^{b}$                          & 1.6  & 1.4                & 0       & 11      \\
\rowcolor{Gray}
Death count for Respiratory Causes (Age $\geq$ 75)$^{b}$    & 1.3  & 1.3                & 0       & 10      \\ \bottomrule        
\end{tabularx}
  \begin{tablenotes}
  \item \footnotesize \textit{Notes}: $^{a}$ 2010-2018 period. $^{b}$ 2008-2015 period.
  \end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/table_matching_distances.tex <==
\begin{table}[h!]
\footnotesize
\caption{Maximum Discrepancies allowed for each Covariate between Treated and Control units}\label{tab2}
\begin{threeparttable}
\begin{tabularx}{\textwidth}{Xcc}
\toprule
& \textbf{\normalsize Hourly} & \textbf{\normalsize Daily} \\ \midrule
\multicolumn{3}{@{}l}{\textbf{\normalsize Calendar Indicators}}\\
\rowcolor{Gray}
Distance in days                               & 20              & 720               \\
Weekday, Bank Days and Holidays in \textit{t}   & 0               & 0              \\
\rowcolor{Gray}
Weekday, Bank Days and Holidays in \textit{t-1} & 0               & 0              \\
Weekday, Bank Days and Holidays in \textit{t-2} & 0               &                \\
\rowcolor{Gray}
Month in \textit{t}                                      &           & 3 \\
\rowcolor{Gray}
\midrule
\multicolumn{3}{@{}l}{\textbf{\normalsize Weather Parameters}}\\
Average Temperature (°C) in \textit{t}                       & 4               & 4              \\
\rowcolor{Gray}
Average Temperature (°C) in \textit{t-1}                     & 4               & 4              \\
Average Temperature (°C) in \textit{t-2}                     & 4               &                \\
\rowcolor{Gray}

Rainfall Dummy in \textit{t}                            & 0               & 0              \\
Rainfall Dummy in \textit{t-1}                         & 0               & 0              \\
\rowcolor{Gray}

Rainfall Dummy in \textit{t-2}                          & 0               &                \\
Average Humidity (\%) in \textit{t}                          & 9               &              \\
\rowcolor{Gray}

Average Humidy (\%) in \textit{t-1}                         & 9               &              \\
Average Humidity (\%) in \textit{t-2}                        & 9               &                \\
\rowcolor{Gray}

Wind direction in two categories (East/West) \textit{t}                  & 0            &  0        \\
Wind direction in two categories (East/West) \textit{t-1}                  & 0            & 0           \\
\rowcolor{Gray}
Wind direction in two categories (East/West) \textit{t-2}                  & 0            &               \\ 
Wind speed in \textit{t}                                & \frac{SD/2}  & 2 \\
\rowcolor{Gray}
Wind speed in \textit{t-1}                               & \frac{SD/2} & 2 \\
Wind speed in \textit{t-2}                               & \frac{SD/2} &  \\
\midrule
\multicolumn{3}{@{}l}{\textbf{\normalsize Health Variables}}\\
\rowcolor{Gray}
Flu epidemic dummy in \textit{t}  & & 0 \\ 
\midrule
\multicolumn{3}{@{}l}{\textbf{\normalsize Vessel Traffic Measures}}\\
\rowcolor{Gray}
Cruise ship gross tonnage in \textit{t-1} & & 30,000 \\ 
Total gross tonnage in \textit{t-1} & & 60,000 \\ 

\bottomrule
\end{tabularx}
\begin{tablenotes}
\footnotesize
\item \textit{Notes}: This table displays the maximum distance allowed for each covariate in the pair matching algorithm. Distances between treated and control units are presented for the hourly and daily experiments. For example, it means that, for each matched pair, treated and control units must have the same values for weekend, days, and holidays indicators in \textit{t}. SD stands for standard deviation. If a discrepancy value is missing, it means that the associated covariate was not used in the matching procedure.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/table_matching_results.tex <==
\begin{table}[h!]
\caption{Number of Matched Pairs by Experiment.}\label{matching_results}
\begin{threeparttable}
\begin{tabularx}{\textwidth}{Xccccc}
\toprule
& \textbf{\shortstack{Hourly \\ cruise arriving}} & \textbf{\shortstack{Hourly \\ cruise departing}} & \textbf{\shortstack{Hourly \\ ferry arriving}} & \textbf{\shortstack{Hourly  \\ ferry departing}} 
& \textbf{\shortstack{Daily \\ cruise}}  \\ \midrule
\rowcolor{Gray}
N$_{\mathrm{Total}}$ &  96,432 & 96,432 & 96,432 & 96,432 & 4,018  \\
N$_{Treated}$ &  4,630   &  4,644  & 12,736  & 12,423  & 932   \\
\rowcolor{Gray}
N$_{\mathrm{Control}}$ & 91,800  & 91,786  & 83,694  & 84,007  & 2,114  \\
N$_{\mathrm{Pairs}}$   & 171 & 156 & 419 & 365 & 58    \\
\bottomrule
\end{tabularx}
\begin{tablenotes}
\footnotesize
\item \textit{Notes}: This table displays the total number of observations, N$_{\mathrm{Total}}$ for each experiment, the number of potential treated and controls units before matching, N$_{\mathrm{Treated}}$ and N$_{\mathrm{Control}}$, and the number of matched pairs, N$_{\mathrm{Pairs}}$.
\end{tablenotes}
\end{threeparttable}
\end{table}
